Detecting Moving Objects With Machine Learning

The scientific study of the Solar System's minor bodies ultimately starts with a search for those bodies. This chapter presents a review of the use of machine learning techniques to find moving objects, both natural and artificial, in astronomical imagery. After a short review of the classical non-machine learning techniques that are historically used, I review the relatively nascent machine learning literature, which can broadly be summarized into three categories: streak detection, detection of moving point sources in image sequences, and detection of moving sources in shift and stack searches. In most cases, convolutional neural networks are utilized, which is the obvious choice given the imagery nature of the inputs. In this chapter I present two example networks: a Residual Network I designed which is in use in various shift and stack searches, and a convolutional neural network that was designed for prediction of source brightnesses and their uncertainties in those same shift-stacks. In discussion of the literature and example networks, I discuss various pitfalls with the use of machine learning techniques, including a discussion on the important issue of overfitting. I discuss various pitfall associated with the use of machine learning techniques, and what I consider best practices to follow in the application of machine learning to a new problem, including methods for the creation of robust training sets, validation, and training to avoid overfitting.

==> titlepage.tex <==
%% Title Page %%
\begin{titlepage}%
  %\begin{titlepagerule}
  %  \title{NA}
  %  %\subtitle{Book Subtitle}
  %  %\volume{2}
  %\end{titlepagerule}

  %\edition{NA}

%  \editedby{Edited by}

  \author{Wesley C. Fraser}
  \address{National Research Council of Canada \\ Herzberg Astronomy and Astrophysics Research Centre \\  5071 W. Saanich Rd., Victoria BC, V9E 2E7, Canada \\ 
  wesley.fraser@nrc-cnrc.gc.ca}

\end{titlepage}

